ResNet After All? Neural ODEs and Their Numerical Solution

A key appeal of the recently proposed Neural Ordinary Differential Equation (ODE) framework is that it seems to provide a continuous-time extension of discrete residual neural networks. As we show herein, though, trained Neural ODE models actually depend on the specific numerical method used during training. If the trained model is supposed to be a flow generated from an ODE, it should be possible to choose another numerical solver with equal or smaller numerical error without loss of performance. We observe that if training relies on a solver with overly coarse discretization, then testing with another solver of equal or smaller numerical error results in a sharp drop in accuracy. In such cases, the combination of vector field and numerical method cannot be interpreted as a flow generated from an ODE, which arguably poses a fatal breakdown of the Neural ODE concept. We observe, however, that there exists a critical step size beyond which the training yields a valid ODE vector field. We propose a method that monitors the behavior of the ODE solver during training to adapt its step size, aiming to ensure a valid ODE without unnecessarily increasing computational cost. We verify this adaptation algorithm on a common bench mark dataset as well as a synthetic dataset.

==> node.tex <==
\section{Problem Setup}

We study the empirical risk minimization (ERM) problem
\begin{equation}\label{eq:erm}
L_\data = \frac{1}{|\data|} \sum_{(x,y) \in \data} l(f(x;w),y)
\end{equation}
where $\data = \{(x_n, y_n)\mid x_n \in \RR^{D_x}, y_n \in \RR^{D_y}, n = 1, \dotsc, N\}$ is a set of training data,
$l : \RR^\Dy \times \RR^\Dy \to \RR$ is a (non-negative) loss function and $f$ is a neural
ODE model, i.e.,
\begin{equation}\label{eq:cont-model}
f = f_d \circ \varphi^{f_v}_T \circ f_u
\end{equation}
where $f_x, x \in \{d, v, u\}$ are (suitable) neural networks
and $\varphi$ is defined to be the flow of the dynamical system
\begin{equation}
\frac{\mathrm{d}z}{\mathrm{d}t} = f_v(z;w_v),\;z(t) = \varphi^{f_v}_t(z(0)).
\end{equation}
As the vector field $f_v$ of the dynamical system is itself defined by a neural network,
evaluating $\varphi_T^{f_v}$ is intractable and we have to resort to a numerical scheme $\Psi$ to
compute $f(z;w)$.
$\Psi$ belongs either to a class of fixed step size $h=TN^{-1}$ methods or is an
adaptive step size solver as proposed in \cite{chen2018neurips}.
For each IVP of the Neural ODE $z_n(0) = f_u(x_n)$, the trajectory computed using a particular solver $\Psi$ is defined as $z_{n,k} = \Psi_h(z_{n,k-1}), k = 1, \dotsc, K$ where $K$ is uniquely defined for fixed-step solvers.


Throughout the paper, we use a fixed step solver to analyze the dynamics of Neural ODEs.
In order to perform some form of gradient descent, reverse-mode auto-differentiation through the solver 
has to be performed.
We choose to back-propagate through the numerical solver and not use the adjoint method described by \cite{chen2018neurips}.
These choices were made, because we want to showcase that the interplay between vector field and ODE solver can lead to discrete dynamics in the simplest settings.
Additionally, using a fixed step solver makes analyzing the problem easy, as the numerical error of the method can be adjusted by simply changing the step size.
For all our experiments we do not use an upstream block $f_u$ similar to the architectures 
proposed in \cite{dupont2019augmented}.
We chose this architecture to increase the impact of the ODE block.
As numerical solvers we use Euler's method, the Midpoint method and a fourth order Runge Kutta method (for more detailed information on Runge Kutta methods see  \cite{hairerWanner})



